Twistor Theory of Higher-Dimensional Black Holes - Part I: Theory

The correspondence between stationary, axisymmetric, asymptotically flat space-times and bundles over a reduced twistor space has been established in four dimensions. The main impediment for an application of this correspondence to examples in higher dimensions has been the lack of a higher-dimensional equivalent of the Ernst potential. This article will propose such a generalized Ernst potential, point out where the rod structure of the space-time can be found in the twistor picture and thereby provide a procedure for generating solutions to the Einstein equations in higher dimensions from the rod structure and other asymptotic data. An important result for the study of five-dimensional examples will be the theorem which relates the patching matrices on the outer semi-infinite rods.

==> headings.tex <==
%% heading style %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%section%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {2.3ex \@plus.2ex}%
                                   {\normalfont\large\bfseries}}
\makeatother

%subsection%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\subsection{\@ifstar\unnumberedsubsection\numberedsubsection}
\def\numberedsubsection{\@ifnextchar[%]
  \numberedsubsectionwithtwoarguments\numberedsubsectionwithoneargument}
\def\unnumberedsubsection{\@ifnextchar[%]
  \unnumberedsubsectionwithtwoarguments\unnumberedsubsectionwithoneargument}
\def\numberedsubsectionwithoneargument#1{\numberedsubsectionwithtwoarguments[#1]{#1}}
\def\unnumberedsubsectionwithoneargument#1{\unnumberedsubsectionwithtwoarguments[#1]{#1}}
\def\numberedsubsectionwithtwoarguments[#1]#2{%
  \ifhmode\par\fi
  \removelastskip
  \vskip 3ex\goodbreak
  \refstepcounter{subsection}%
  \noindent
  \leavevmode
  \begingroup
  \bfseries \indent
  \thesubsection\ 
  #2. 
  \endgroup
  \addcontentsline{toc}{subsection}{%
    \protect\numberline{\thesubsection}%
    #1}%
  }
\def\unnumberedsubsectionwithtwoarguments[#1]#2{%
  \ifhmode\par\fi
  \removelastskip
  \vskip 3ex\goodbreak
%  \refstepcounter{section}%
  \noindent
  \leavevmode
  \begingroup
  \bfseries \indent
%  \thesubsection\ 
  #2.
  \endgroup
%  \addcontentsline{toc}{subsection}{%
%    \protect\numberline{\thesection}%
%    #1}%
  }
\makeatother


%subsubsection%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\subsubsection{\@ifstar\unnumberedsubsubsection\numberedsubsubsection}
\def\numberedsubsubsection{\@ifnextchar[%]
  \numberedsubsubsectionwithtwoarguments\numberedsubsubsectionwithoneargument}
\def\unnumberedsubsubsection{\@ifnextchar[%]
  \unnumberedsubsubsectionwithtwoarguments\unnumberedsubsubsectionwithoneargument}
\def\numberedsubsubsectionwithoneargument#1{\numberedsubsubsectionwithtwoarguments[#1]{#1}}
\def\unnumberedsubsubsectionwithoneargument#1{\unnumberedsubsubsectionwithtwoarguments[#1]{#1}}
\def\numberedsubsubsectionwithtwoarguments[#1]#2{%
  \ifhmode\par\fi
  \removelastskip
  \vskip 2ex\goodbreak
  \refstepcounter{subsubsection}%
  \noindent
  \leavevmode
  \begingroup
  \itshape \indent
  \thesubsubsection\ 
  #2.
  \endgroup
  \addcontentsline{toc}{subsubsection}{%
    \protect\numberline{\thesubsubsection}%
    #1}%
  }
\def\unnumberedsubsubsectionwithtwoarguments[#1]#2{%
  \ifhmode\par\fi
  \removelastskip
  \vskip 2ex\goodbreak
%  \refstepcounter{section}%
  \noindent
  \leavevmode
  \begingroup
  \itshape \indent
%  \thesubsubsection\ 
  #2.  
  \endgroup
%  \addcontentsline{toc}{subsubsection}{%
%    \protect\numberline{\thesubsubsection}%
%    #1}%
  }
\makeatother

%% ToC style %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\contentsnamefont{\large\bfseries}

\newcommand{\mycftdotsep}{5.5}
\newcommand{\mycftdotfill}[1]{%
  \leaders\hbox{$\mkern #1 mu\hbox{.}\mkern #1 mu$}\hfill}
  
%% defines whether the sections are in bold or note
%% \bfseries = in bold, \mdseries = not bold
\newcommand{\Myseries}{\mdseries}

\makeatletter
\def\l@part{\@tocline{-1}{3pt plus1pt}{1pc}{}{\bfseries}}  
\def\appendixname{} 
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\@M
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax \advance\leftskip\@tempdima\relax
    \rightskip\@pnumwidth plus4em \parfillskip-\@pnumwidth
    #5\leavevmode\hskip-\@tempdima #6\nobreak\relax
    \ifnum#1<1\hfill\else \mycftdotfill{\mycftdotsep} 
		\fi\hbox  to\@pnumwidth{\ifnum#1<2\@tocpagenumBF{#7\hspace{1.2em}}\else\@tocpagenum{#7\hspace{1.2em}}\fi}\par
    \nobreak
    \endgroup
  \fi}
  \def\@tocpagenumBF#1{\hss{\Myseries #1}}
  \renewcommand{\tocsection}[3]{%
    \indentlabel{\@ifnotempty{#2}{\Myseries\ignorespaces#1 \makebox[1.0em][l]{#2.} }}\Myseries #3}
  \def\l@subsection{\@tocline{2}{0pt}{2.3pc}{5pc}{}}
  \renewcommand{\tocsubsection}[3]{%
    \indentlabel{\@ifnotempty{#2}{\ignorespaces#1 \makebox[1.7em][l]{#2.} }}\mdseries #3}
  \def\l@subsubsection{\@tocline{3}{0pt}{4pc}{7pc}{}} %%%  2.3pc or 4.0pc
  \renewcommand{\tocsubsubsection}[3]{%
    \indentlabel{\@ifnotempty{#2}{\ignorespaces#1 \makebox[2.5em][l]{#2.} }}\mdseries #3}
\makeatother

%%% citestyle %%%%%%%%%%%%%%%%%%%%
\def\citeform#1{{\mdseries#1}}

